Cash Accumulation Strategy based on Optimal Replication of Random Claims with Ordinary Integrals

This paper presents a numerical model to solve the problem of cash accumulation strategies for products with an unknown future price, like assets. Stock prices are modeled by a discretized Wiener Process, and by the means of ordinary integrals this Wiener Process will be exactly matched at a preset terminal time. Three applications of the model are presented: accumulating cash for a single asset, for set of different assets, and for a proportion of the excess achieved by a certain asset. Furthermore, an analysis of the efficiency of the model as function of different parameters is performed.

==> guide/guide.tex <==

\section*{Nomenclature}

\begin{tabbing}
  XXX \= \kill% this line sets tab stop
  $J$ \> Jacobian Matrix \\
  $f$ \> Residual value vector \\
  $x$ \> Variable value vector \\
  $F$ \> Force, N \\
  $m$ \> Mass, kg \\
  $\Delta x$ \> Variable displacement vector \\
  $\alpha$ \> Acceleration, m/s\textsuperscript{2} \\[5pt]
  \textit{Subscript}\\
  $i$ \> Variable number \\
 \end{tabbing}

\section{Introduction}

This would be a good place to insert some text that make sense relative
to the paper being written.
Of course, for example purposes, the text is quite meaningless.

\subsection{Background}

This background section is here only to demonstrate \verb|\subsection|
usage.
And following this, the next section level will need to be demonstrated.

\subsubsection{Detail}

Here is a \verb|\subsubsection| that would normally come in pairs of two
according to the requirements of an outline, but for the sake of
demonstration, we are only showing a single \verb|\subsubsection|.

\section{Model}

We should probably include some math.
Here we begin with Eq.~(\ref{e:function}) that demonstrates some math
typesetting.
\begin{equation}
 \label{e:function}
 \int_{0}^{r_{2}} F(r,\varphi) \, dr \, d\varphi =
    \left[ \sigma r_{2}/(2\mu_{0}) \right] \cdot
    \int_{0}^{\infty} \exp(-\rho|z_{j}-z_{i}|) \, \lambda^{-1} 
\end{equation}
Eq.~(\ref{e:function}) is grand.
Some say it is due to Rebek.\cite{rebek:82bk}

\section{Results}

In this section we will introduce some figures and tables.
It can be seen in figure~\ref{f:magnetic_field} that magnetization is a
function of applied field.
\begin{figure}[htb]% order of placement preference: here, top, bottom
 \includegraphics{figure_magnet}
 \caption{Magnetization as a function of applied field, which has
   borders so thick that they overwhelm the data and for some reason the
   ordinate label is rotated 90 degrees to make it difficult to
   read. This figure also demonstrates the dangers of using a bitmap
   as opposed to a vector image.}
 \label{f:magnetic_field}
\end{figure}
Sometimes writing meaningless text can be quiet easy, but other times
one is hard pressed to keep the words flowing.\footnote{And sometimes
things get carried away in endless detail.}
Meanwhile back in the other world, table~\ref{t:scheme_comparison} shows
a nifty comparison.
\begin{table}% no placement specified: defaults to here, top, bottom, page
 \begin{center}
  \caption{Variable and Fixed Coefficient Runge-Kutta Schemes as a
           Function of Reynolds Number}
  \label{t:scheme_comparison}
  \begin{tabular}{rrr}
       Re & Vary & Fixed \\\hline
        1 &  868 & 4,271 \\
       10 &  422 & 2,736 \\
       25 &  252 & 1,374 \\
       50 &  151 &   736 \\
      100 &  110 &   387 \\
      500 &   85 &   136 \\
    1,000 &   77 &   117 \\
    5,000 &   81 &    98 \\
   10,000 &   82 &    99
  \end{tabular}
 \end{center}
\end{table}

\section{Conclusion}

After much typing, the paper can now conclude.
Four rocks were next to the channel.
This caused a few standing waves during the rip that one could ride on
the way in or jump on the way out.

\section*{Appendix}

An appendix, if needed, should appear before the acknowledgments.
Use the 'starred' version of the \verb|\section| commands to avoid
section numbering.

\section*{Acknowledgments}

A place to recognize others.

\begin{thebibliography}{9}% maximum number of references (for label width)
 \bibitem{rebek:82bk}
 Rebek, A., {\it Fickle Rocks}, Fink Publishing, Chesapeake, 1982.
\end{thebibliography}


% - Release $Name:  $ -


==> sections/acknowledgements.tex <==
\section*{Acknowledgements}

Special thanks to Nikolai Dokuchaev, for his assistance for providing the equations for the model, assisting when generating the model, and supervising this project in general.


==> sections/appendices.tex <==
\section*{Appendices}

\begin{lstlisting}[frame=none]
clear 
% Define end of time interval
T=1;
N = 365;
dt = T/N;
%Define number of dimensions
m = 2;

W = zeros(m,N);
dW = zeros(m,N);
x= zeros(m,N); 

if m == 1
    W0 = 150;
    a = @(z) 0;
    sigma = @(z)0.5;
    start = 50;
end

if m ==2
    W0 = [200;
        400];
    a = @(z) [0;
        0];    
    sigma = @(z) 1;
    start = [20,
        20];
end

a = @(z) 0;
sigma =  @(z)0.5;
for i=1:N
    if i ==1 
        dW(:,1) = W0 .*( a(i*dt) .* dt + sigma(i*dt) .* sqrt(dt) .* randn(m,1));
        W(:,1) = W0 + dW(:,1);
    else
        dW(:,i) = W(:,i-1) .*( a(i*dt).* dt+  sigma(i*dt) .*  sqrt(dt).*randn(m,1));
        W(:,i) = W(:,i-1) + dW(:,i); 
    end
end

Gamma = @(t)1; 
ir = 0.3;
A = ir;
Q= @(x) exp(2*A*(T-x)).*Gamma(x).^(-1); 
R = @(s) quad(Q,s,T); 
M = 0;

for q = 1:N
    t = q*dt;
    r = R(t);
    M = M + r.^(-1) * dW(:,q);
    mu = R(0).^(-1)*(W0 - exp(A*T).*start) + M;
    u = Gamma(t).^(-1)*exp(A*(T-t))*mu;
    if q == 1
        x(:,1) = exp(ir*dt).*(start + u*dt);
    else
        x(:,q) = (x(:,q-1) + u*dt).*exp(ir*dt);
    end
end   
figure
if m==1
    plot( 0:dt:T, [W0,W]) 
    hold on
    plot( 0:dt:T, [start, x])
else
    plot(0:dt:T, [sum(W0), sum(W)])
    hold on
    plot( 0:dt:T, [sum(start), sum(x)])
end
hold on
xlabel('Time (years)')
ylabel('Value ($)')
legend( 'Stock Price', 'Accumulated Cash')
matlab2tikz('21.tex')

if m == 2
    figure
    plot( 0:dt:T, [W0(1),W(1,:)] )
    hold on 
    plot( 0:dt:T, [W0(2),W(2,:)], 'black')
    xlabel('Time (years)')
    ylabel('Dollars ($)')
    legend('Stock Price 1', 'Stock Price 2')
end


\end{lstlisting}


\begin{lstlisting}[frame=none]
clear 
% Define end of time interval
T=2;
N = 365;
dt = T/N;
m=1;

%Define arrays for simulation of process
W = zeros(m,N);
dW = zeros(m,N);
x= zeros(m,N); 
f= zeros(m,N);

W0 = 75;
a = @(z) 0;
sigma = 0.3;
i=1;
dW(:,1) = W0 .*( a(i*dt) .* dt + sigma .* sqrt(dt) .* randn(m,1));
W(:,1) = W0 + dW(:,1);
for i=2:N
    dW(:,i) = W(:,i-1) .*( a(i*dt).* dt+  sigma .*  sqrt(dt).*randn(m,1));
    W(:,i) = W(:,i-1) + dW(:,i);     
end

Gamma = @(t)1; %@(z) (T-z).^0.5;
r = 0.03;
c = 0.5;
A = r;
K = 30;
Q= @(x) exp(2*A*(T-x)).*Gamma(x).^(-1); 
R = @(s) quad(Q,s,T); 
M=0;
d1 = @(q) (log(W(q)/K) + (T-q*dt)*(r+sigma.^2/2))/(sigma*sqrt(T-q*dt));
d2 = @(q) d1(q) - sigma*sqrt(T-q*dt);

d10 = (log(W0/K) + (T)*(r+sigma.^2/2))/(sigma*sqrt(T)) ;
d20 = d10 - sigma*sqrt(T);
H0 = normcdf(d10)*W0 - normcdf(d20)*K*exp(-r*T);


for q = 1:N
    df = normcdf(d1(q))*sigma*dW(:,q);
    if q == 1
        f(:,q) = max(H0 + df,0);
    else
        f(:,q) = max(f(:,q-1) + df,0);
    end
    
    t = q*dt;
    M = M + R(t).^(-1)* df;
    mu = R(0).^(-1)*(H0 ) + M;
    u = c*Gamma(t).^(-1)*exp(A*(T-t))*mu;
    if q==1
        x(:,q) = exp(r*dt).*(u*dt);
    else 
        x(:,q) = (x(:,q-1) + u*dt).*exp(r*dt);
    end

end   

figure
plot(0:dt:T, c*[H0,f]);
hold on
plot(0:dt:T, [0,x]);
xlabel('Time (years)')
ylabel('Value ($)')
legend( 'Equity Excess', 'Accumulated Cash')

\end{lstlisting}
